Memory-Sample Lower Bounds for Learning with Classical-Quantum Hybrid Memory

In a work by Raz (J. ACM and FOCS 16), it was proved that any algorithm for parity learning on $n$ bits requires either $\Omega(n^2)$ bits of classical memory or an exponential number (in~$n$) of random samples. A line of recent works continued that research direction and showed that for a large collection of classical learning tasks, either super-linear classical memory size or super-polynomially many samples are needed. However, these results do not capture all physical computational models, remarkably, quantum computers and the use of quantum memory. It leaves the possibility that a small piece of quantum memory could significantly reduce the need for classical memory or samples and thus completely change the nature of the classical learning task. In this work, we prove that any quantum algorithm with both, classical memory and quantum memory, for parity learning on $n$ bits, requires either $\Omega(n^2)$ bits of classical memory or $\Omega(n)$ bits of quantum memory or an exponential number of samples. In other words, the memory-sample lower bound for parity learning remains qualitatively the same, even if the learning algorithm can use, in addition to the classical memory, a quantum memory of size $c n$ (for some constant $c>0$). Our results refute the possibility that a small amount of quantum memory significantly reduces the size of classical memory needed for efficient learning on these problems. Our results also imply improved security of several existing cryptographical protocols in the bounded-storage model (protocols that are based on parity learning on $n$ bits), proving that security holds even in the presence of a quantum adversary with at most $c n^2$ bits of classical memory and $c n$ bits of quantum memory (for some constant $c>0$).

==> lemma3-2.tex <==
	\begin{lemma}
		For every orthogonal projections $\Pi$, we have
		\[\TrN[2]{\rho\mt_{XV}-\big(\id\mt_X\otimes \Pi\big)\rho\mt_{XV}\big(\id\mt_X\otimes \Pi\big)}\leq 4-4w\big(\Pi,\rho\mt_{XV}\big)^2\]
	\end{lemma}
	\begin{proof}
		By Fuchs-van de Graaf inequality, it suffices to prove the following bound on fidelity:
		\[F\left(\rho\mt_{XV},\big(\id\mt_X\otimes \Pi\big)\rho\mt_{XV}\big(\id\mt_X\otimes \Pi\big)\right)\geq w\big(\Pi,\rho\mt_{XV}\big)^2.\]
		Suppose $u\in\{0,1\}^n\otimes\mathcal{H}\otimes\mathcal{H}\mt_A$ is a purification of $\rho\mt_{XV}$, that is,
		$\rho\mt_{XV}=\Tr\mt_A[uu\ct]$. Then $\big(\id\mt_X\otimes\Pi\otimes\id\mt_A\big)u$ is a purification of $\big(\id\mt_X\otimes \Pi\big)\rho\mt_{XV}\big(\id\mt_X\otimes \Pi\big)$. By Uhlmann's theorem we have
		\begin{align*} 
			F\left(\rho\mt_{XV},\big(\id\mt_X\otimes \Pi\big)\rho\mt_{XV}\big(\id\mt_X\otimes \Pi\big)\right)
			&\geq \left|u\ct\big(\id\mt_X\otimes\Pi\otimes\id\mt_A\big)u\right|^2 \\
			&=\Tr\left[\big(\id\mt_X\otimes\Pi\otimes\id\mt_A\big)uu\ct\right]^2 \\
			&=\Tr\left[\big(\id\mt_X\otimes\Pi\big) \Tr\mt_A[uu\ct]\right]^2 \\
			&=w\big(\Pi,\rho\mt_{XV}\big)^2. \qedhere
		\end{align*}
	\end{proof}

